Towards Evology: a Market Ecology Agent-Based Model of US Equity Mutual Funds

The profitability of various investment styles in investment funds depends on macroeconomic conditions. Market ecology, which views financial markets as ecosystems of diverse, interacting and evolving trading strategies, has shown that endogenous interactions between strategies determine market behaviour and styles' performance. We present Evology: a heterogeneous, empirically calibrated multi-agent market ecology agent-based model to quantify endogenous interactions between US equity mutual funds, particularly Value and Growth investment styles. We outline the model design, validation and calibration approach and its potential for optimising investment strategies using machine learning algorithms.

==> abstract.tex <==
Market ecology views financial markets as ecosystems of diverse, interacting and evolving trading strategies. We present a heterogeneous, empirically calibrated multi-agent market ecology agent-based model. We outline its potential as a valuable and challenging training ground for optimising trading and investment strategies using machine learning algorithms.
